SynDistNet: Self-Supervised Monocular Fisheye Camera Distance Estimation Synergized with Semantic Segmentation for Autonomous Driving

State-of-the-art self-supervised learning approaches for monocular depth estimation usually suffer from scale ambiguity. They do not generalize well when applied on distance estimation for complex projection models such as in fisheye and omnidirectional cameras. This paper introduces a novel multi-task learning strategy to improve self-supervised monocular distance estimation on fisheye and pinhole camera images. Our contribution to this work is threefold: Firstly, we introduce a novel distance estimation network architecture using a self-attention based encoder coupled with robust semantic feature guidance to the decoder that can be trained in a one-stage fashion. Secondly, we integrate a generalized robust loss function, which improves performance significantly while removing the need for hyperparameter tuning with the reprojection loss. Finally, we reduce the artifacts caused by dynamic objects violating static world assumptions using a semantic masking strategy. We significantly improve upon the RMSE of previous work on fisheye by 25% reduction in RMSE. As there is little work on fisheye cameras, we evaluated the proposed method on KITTI using a pinhole model. We achieved state-of-the-art performance among self-supervised methods without requiring an external scale estimation.

==> bib/backup.tex <==
@inproceedings{yogamani2019woodscape,
	title        = {{Woodscape: A Multi-Task, Multi-Camera Fisheye Dataset for Autonomous Driving}},
	author       = {Yogamani, Senthil and Hughes, Ciar{\'a}n and Horgan, Jonathan and Sistu, Ganesh and Varley, Padraig and O'Dea, Derek and Uric{\'a}r, Michal and Milz, Stefan and Simon, Martin and Amende, Karl and others},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {9308--9318}
}
@article{geiger2013vision,
	title        = {{Vision Meets Robotics: The KITTI Dataset}},
	author       = {Geiger, Andreas and Lenz, Philip and Stiller, Christoph and Urtasun, Raquel},
	year         = 2013,
	journal      = {The International Journal of Robotics Research},
	volume       = 32,
	number       = 11,
	pages        = {1231--1237}
}
@article{conrady1919decentred,
	title        = {Decentred lens-systems},
	author       = {Conrady, Alexander Eugen},
	year         = 1919,
	journal      = {Monthly notices of the royal astronomical society},
	publisher    = {The Royal Astronomical Society},
	volume       = 79,
	number       = 5,
	pages        = {384--390}
}
@inproceedings{uricar2019desoiling,
	title        = {Desoiling Dataset: Restoring Soiled Areas on Automotive Fisheye Cameras},
	author       = {Uric{\'a}r, Michal and Ulicny, Jan and Sistu, Ganesh and Rashed, Hazem and Krizek, Pavel and Hurych, David and Vobecky, Antonin and Yogamani, Senthil},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE International Conference on Computer Vision Workshops},
	pages        = {0--0}
}
@inproceedings{horgan2015vision,
	title        = {Vision-based driver assistance systems: Survey, taxonomy and advances},
	author       = {Horgan, Jonathan and Hughes, Ciar{\'a}n and McDonald, John and Yogamani, Senthil},
	year         = 2015,
	booktitle    = {2015 IEEE 18th International Conference on Intelligent Transportation Systems},
	pages        = {2032--2039},
	organization = {IEEE}
}
@article{sistu2019real,
	title        = {Real-time joint object detection and semantic segmentation network for automated driving},
	author       = {Sistu, Ganesh and Leang, Isabelle and Yogamani, Senthil},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1901.03912}
}
@article{tripathi2020trained,
	title        = {Trained Trajectory based Automated Parking System using Visual SLAM},
	author       = {Tripathi, Nivedita and Sistu, Ganesh and Yogamani, Senthil},
	year         = 2020,
	journal      = {arXiv preprint arXiv:2001.02161}
}
@inproceedings{uvrivcavr2019soilingnet,
	title        = {SoilingNet: Soiling Detection on Automotive Surround-View Cameras},
	author       = {U{\v{r}}i{\v{c}}{\'a}{\v{r}}, Michal and K{\v{r}}{\'\i}{\v{z}}ek, Pavel and Sistu, Ganesh and Yogamani, Senthil},
	year         = 2019,
	booktitle    = {2019 IEEE Intelligent Transportation Systems Conference (ITSC)},
	pages        = {67--72},
	organization = {IEEE}
}
@inproceedings{dahal2019deeptrailerassist,
	title        = {DeepTrailerAssist: Deep Learning based trailer detection, tracking and articulation angle estimation on automotive rear-view camera},
	author       = {Dahal, Ashok and Hossen, Jakir and Sumanth, Chennupati and Sistu, Ganesh and Malhan, Kazumi and Amasha, Muhammad and Yogamani, Senthil},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE International Conference on Computer Vision Workshops},
	pages        = {0--0}
}
@article{heimberger2017computer,
	title        = {Computer vision in automated parking systems: Design, implementation and challenges},
	author       = {Heimberger, Markus and Horgan, Jonathan and Hughes, Ciar{\'a}n and McDonald, John and Yogamani, Senthil},
	year         = 2017,
	journal      = {Image and Vision Computing},
	publisher    = {Elsevier},
	volume       = 68,
	pages        = {88--101}
}
@inproceedings{Guizilini2020a,
	title        = {{3D Packing for Self-Supervised Monocular Depth Estimation}},
	author       = {Guizilini, Vitor and Ambrus, Rares and Pillai, Sudeep and Gaidon, Adrien},
	year         = 2020,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Seattle, WA, USA},
	pages        = {2485--2494}
}
@article{yahiaoui2019fisheyemodnet,
	title        = {Fisheyemodnet: Moving object detection on surround-view cameras for autonomous driving},
	author       = {Yahiaoui, Marie and Rashed, Hazem and Mariotti, Letizia and Sistu, Ganesh and Clancy, Ian and Yahiaoui, Lucie and Kumar, Varun Ravi and Yogamani, Senthil},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1908.11789}
}
@inproceedings{drulea2014omnidirectional,
	title        = {Omnidirectional stereo vision using fisheye lenses},
	author       = {Drulea, Marius and Szakats, Istvan and Vatavu, Andrei and Nedevschi, Sergiu},
	year         = 2014,
	booktitle    = {2014 IEEE 10th International Conference on Intelligent Computer Communication and Processing (ICCP)},
	pages        = {251--258},
	organization = {IEEE}
}
@inproceedings{decamp2010immersive,
	title        = {An immersive system for browsing and visualizing surveillance video},
	author       = {DeCamp, Philip and Shaw, George and Kubat, Rony and Roy, Deb},
	year         = 2010,
	booktitle    = {Proceedings of the 18th ACM international conference on Multimedia},
	pages        = {371--380},
	organization = {ACM}
}
@inproceedings{Godard2019,
	title        = {{Digging Into Self-Supervised Monocular Depth Estimation}},
	author       = {Godard, Cl{\'e}ment and Mac Aodha, Oisin and Firman, Michael and Brostow, Gabriel J.},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {3828--3838},
	keywords     = {Depth Prediction}
}
@inproceedings{Eigen_14,
	title        = {{Depth Map Prediction from a Single Image Using a Multi-Scale Deep Network}},
	author       = {Eigen, David and Puhrsch, Christian and Fergus, Rob},
	year         = 2014,
	month        = dec,
	booktitle    = {Proc. of NIPS},
	address      = {Montr\' {e}al, QC, Canada},
	pages        = {2366--2374},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{caruso2015large,
	title        = {Large-scale direct slam for omnidirectional cameras},
	author       = {Caruso, David and Engel, Jakob and Cremers, Daniel},
	year         = 2015,
	booktitle    = {2015 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
	pages        = {141--148},
	organization = {IEEE}
}
@inproceedings{varun18,
	title        = {Monocular fisheye camera depth estimation using sparse lidar supervision},
	author       = {Kumar, Varun Ravi and Milz, Stefan and Witt, Christian and Simon, Martin and Amende, Karl and Petzold, Johannes and Yogamani, Senthil and Pech, Timo},
	year         = 2018,
	booktitle    = {2018 21st International Conference on Intelligent Transportation Systems (ITSC)},
	pages        = {2853--2858},
	organization = {IEEE}
}
@inproceedings{zioulis2018omnidepth,
	title        = {Omnidepth: Dense depth estimation for indoors spherical panoramas},
	author       = {Zioulis, Nikolaos and Karakottas, Antonis and Zarpalas, Dimitrios and Daras, Petros},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {448--465}
}
@inproceedings{shah1994depth,
	title        = {Depth estimation using stereo fish-eye lenses},
	author       = {Shah, Shishir and Aggarwal, JK},
	year         = 1994,
	booktitle    = {Proceedings of 1st International Conference on Image Processing},
	volume       = 2,
	pages        = {740--744},
	organization = {IEEE}
}
@inproceedings{zhou2017unsupervised,
	title        = {Unsupervised learning of depth and ego-motion from video},
	author       = {Zhou, Tinghui and Brown, Matthew and Snavely, Noah and Lowe, David G},
	year         = 2017,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {1851--1858}
}
@article{li2008binocular,
	title        = {Binocular spherical stereo},
	author       = {Li, Shigang},
	year         = 2008,
	journal      = {IEEE Transactions on intelligent transportation systems},
	publisher    = {IEEE},
	volume       = 9,
	number       = 4,
	pages        = {589--600}
}
@article{ma20153d,
	title        = {3D reconstruction from full-view fisheye camera},
	author       = {Ma, Chuiwen and Shi, Liang and Huang, Hanlu and Yan, Mengyuan},
	year         = 2015,
	journal      = {arXiv preprint arXiv:1506.06273}
}
@inproceedings{pathak2016dense,
	title        = {Dense 3D reconstruction from two spherical images via optical flow-based equirectangular epipolar rectification},
	author       = {Pathak, Sarthak and Moro, Alessandro and Yamashita, Atsushi and Asama, Hajime},
	year         = 2016,
	booktitle    = {2016 IEEE International Conference on Imaging Systems and Techniques (IST)},
	pages        = {140--145},
	organization = {IEEE}
}
@inproceedings{li2005spherical,
	title        = {Spherical stereo for the construction of immersive VR environment},
	author       = {Li, Shigang and Fukumori, Kiyotaka},
	year         = 2005,
	booktitle    = {IEEE Proceedings. VR 2005. Virtual Reality, 2005.},
	pages        = {217--222},
	organization = {IEEE}
}
@inproceedings{huang20176,
	title        = {6-DOF VR videos with a single 360-camera},
	author       = {Huang, Jingwei and Chen, Zhili and Ceylan, Duygu and Jin, Hailin},
	year         = 2017,
	booktitle    = {2017 IEEE Virtual Reality (VR)},
	pages        = {37--44},
	organization = {IEEE}
}
@inproceedings{facil2019cam,
	title        = {CAM-Convs: camera-aware multi-scale convolutions for single-view depth},
	author       = {Facil, Jose M and Ummenhofer, Benjamin and Zhou, Huizhong and Montesano, Luis and Brox, Thomas and Civera, Javier},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages        = {11826--11835}
}
@inproceedings{yadati2017multiscale,
	title        = {Multiscale two-view stereo using convolutional neural networks for unrectified images},
	author       = {Yadati, Pramod and Namboodiri, Anoop M},
	year         = 2017,
	booktitle    = {2017 Fifteenth IAPR International Conference on Machine Vision Applications (MVA)},
	pages        = {346--349},
	organization = {IEEE}
}
@inproceedings{usenko2018double,
	title        = {The double sphere camera model},
	author       = {Usenko, Vladyslav and Demmel, Nikolaus and Cremers, Daniel},
	year         = 2018,
	booktitle    = {2018 International Conference on 3D Vision (3DV)},
	pages        = {552--560},
	organization = {IEEE}
}
@article{roxas2019real,
	title        = {Real-Time Variational Fisheye Stereo without Rectification and Undistortion},
	author       = {Roxas, Menandro and Oishi, Takeshi},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1909.07545}
}
@book{hartley2003multiple,
	title        = {Multiple view geometry in computer vision},
	author       = {Hartley, Richard and Zisserman, Andrew},
	year         = 2003,
	publisher    = {Cambridge university press}
}
@article{franke1998autonomous,
	title        = {Autonomous driving goes downtown},
	author       = {Franke, Uwe and Gavrila, Dariu and Gorzig, Steffen and Lindner, Frank and Puetzold, F and Wohler, Christian},
	year         = 1998,
	journal      = {IEEE Intelligent Systems and Their Applications},
	publisher    = {IEEE},
	volume       = 13,
	number       = 6,
	pages        = {40--48}
}
@article{meijering2002chronology,
	title        = {A chronology of interpolation: from ancient astronomy to modern signal and image processing},
	author       = {Meijering, Erik},
	year         = 2002,
	journal      = {Proceedings of the IEEE},
	publisher    = {IEEE},
	volume       = 90,
	number       = 3,
	pages        = {319--342}
}
@inproceedings{shi2016real,
	title        = {Real-time single image and video super-resolution using an efficient sub-pixel convolutional neural network},
	author       = {Shi, Wenzhe and Caballero, Jose and Husz{\'a}r, Ferenc and Totz, Johannes and Aitken, Andrew P and Bishop, Rob and Rueckert, Daniel and Wang, Zehan},
	year         = 2016,
	booktitle    = {Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages        = {1874--1883}
}
@article{odena2016deconvolution,
	title        = {Deconvolution and checkerboard artifacts},
	author       = {Odena, Augustus and Dumoulin, Vincent and Olah, Chris},
	year         = 2016,
	journal      = {Distill},
	volume       = 1,
	number       = 10,
	pages        = {e3}
}
@inproceedings{pinard2018learning,
	title        = {Learning structure-from-motion from motion},
	author       = {Pinard, Cl{\'e}ment and Chevalley, Laure and Manzanera, Antoine and Filliat, David},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {0--0}
}
@article{zhou2018unsupervised,
	title        = {Unsupervised Learning of Monocular Depth Estimation with Bundle Adjustment, Super-Resolution and Clip Loss},
	author       = {Zhou, Lipu and Ye, Jiamin and Abello, Montiel and Wang, Shengze and Kaess, Michael},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1812.03368}
}
@article{plagemann2010nonparametric,
	title        = {A nonparametric learning approach to range sensing from omnidirectional vision},
	author       = {Plagemann, Christian and Stachniss, Cyrill and Hess, J{\"u}rgen and Endres, Felix and Franklin, Nathan},
	year         = 2010,
	journal      = {Robotics and Autonomous Systems},
	publisher    = {Elsevier},
	volume       = 58,
	number       = 6,
	pages        = {762--772}
}
@article{ruder2018artistic,
	title        = {Artistic style transfer for videos and spherical images},
	author       = {Ruder, Manuel and Dosovitskiy, Alexey and Brox, Thomas},
	year         = 2018,
	journal      = {International Journal of Computer Vision},
	publisher    = {Springer},
	volume       = 126,
	number       = 11,
	pages        = {1199--1219}
}
@article{monroy2018salnet360,
	title        = {Salnet360: Saliency maps for omni-directional images with cnn},
	author       = {Monroy, Rafael and Lutz, Sebastian and Chalasani, Tejo and Smolic, Aljosa},
	year         = 2018,
	journal      = {Signal Processing: Image Communication},
	publisher    = {Elsevier},
	volume       = 69,
	pages        = {26--34}
}
@inproceedings{frossard2017graph,
	title        = {Graph-based classification of omnidirectional images},
	author       = {Frossard, Pascal and Khasanova, Renata},
	year         = 2017,
	booktitle    = {2017 IEEE International Conference on Computer Vision Workshops (ICCVW)},
	pages        = {860--869},
	organization = {IEEE}
}
@inproceedings{su2017learning,
	title        = {Learning spherical convolution for fast features from 360 imagery},
	author       = {Su, Yu-Chuan and Grauman, Kristen},
	year         = 2017,
	booktitle    = {Advances in Neural Information Processing Systems},
	pages        = {529--539}
}
@inproceedings{jeon2017active,
	title        = {Active convolution: Learning the shape of convolution for image classification},
	author       = {Jeon, Yunho and Kim, Junmo},
	year         = 2017,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {4201--4209}
}
@inproceedings{dai2017deformable,
	title        = {Deformable convolutional networks},
	author       = {Dai, Jifeng and Qi, Haozhi and Xiong, Yuwen and Li, Yi and Zhang, Guodong and Hu, Han and Wei, Yichen},
	year         = 2017,
	booktitle    = {Proceedings of the IEEE international conference on computer vision},
	pages        = {764--773}
}
@article{deng2018restricted,
	title        = {Restricted deformable convolution based road scene semantic segmentation using surround view cameras},
	author       = {Deng, Liuyuan and Yang, Ming and Li, Hao and Li, Tianyi and Hu, Bing and Wang, Chunxiang},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1801.00708}
}
@inproceedings{tateno2018distortion,
	title        = {Distortion-aware convolutional filters for dense prediction in panoramic images},
	author       = {Tateno, Keisuke and Navab, Nassir and Tombari, Federico},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {707--722}
}
@inproceedings{garg2016unsupervised,
	title        = {{Unsupervised CNN for Single View Depth Estimation: Geometry to the Rescue}},
	author       = {Garg, Ravi and BG, Vijay Kumar and Carneiro, Gustavo and Reid, Ian},
	year         = 2016,
	month        = oct,
	booktitle    = {Proc. of ECCV},
	address      = {Amsterdam, The Netherlands},
	pages        = {740--756},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{jaderberg2015spatial,
	title        = {Spatial transformer networks},
	author       = {Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and others},
	year         = 2015,
	booktitle    = {Advances in neural information processing systems},
	pages        = {2017--2025}
}
@article{wang2004image,
	title        = {{Image Quality Assessment: From Error Visibility to Structural Similarity}},
	author       = {Wang, Zhou and Bovik, Alan Conrad and Sheikh, Hamid Rahim and Simoncelli, Eero P.},
	year         = 2004,
	month        = apr,
	journal      = {IEEE Trans. on Image Processing},
	publisher    = {IEEE},
	volume       = 13,
	number       = 4,
	pages        = {600--612}
}
@inproceedings{ummenhofer2017demon,
	title        = {Demon: Depth and motion network for learning monocular stereo},
	author       = {Ummenhofer, Benjamin and Zhou, Huizhong and Uhrig, Jonas and Mayer, Nikolaus and Ilg, Eddy and Dosovitskiy, Alexey and Brox, Thomas},
	year         = 2017,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {5038--5047}
}
@inproceedings{mahjourian2018unsupervised,
	title        = {{Unsupervised Learning of Depth and Ego-Motion from Monocular Video Using 3D Geometric Constraints}},
	author       = {Mahjourian, Reza and Wicke, Martin and Angelova, Anelia},
	year         = 2018,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Salt Lake City, UT, USA},
	pages        = {5667--5675},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{Wang2019,
	title        = {{Recurrent Neural Network for (Un-)Supervised Learning of Monocular Video Visual Odometry and Depth}},
	author       = {Wang, Rui and Pizer, Stephen M. and Frahm, Jan-Michael},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {5555--5564},
	keywords     = {Speech Recognition}
}
@inproceedings{Zhang2019c,
	title        = {{Exploiting Temporal Consistency for Real-Time Video Depth Estimation}},
	author       = {Zhang, Haokui and Shen, Chunhua and Li, Ying and Cao, Yuanzhouhan and Liu, Yu and Yan, Youliang},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {1725--1734},
	keywords     = {Depth Prediction}
}
@inproceedings{Gordon2019,
	title        = {{Depth from Videos in the Wild: Unsupervised Monocular Depth Learning from Unknown Cameras}},
	author       = {Gordon, Ariel and Li, Hanhan and Jonschkowski, Rico and Angelova, Anelia},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {8977--8986},
	keywords     = {Depth Prediction}
}
@inproceedings{Aleotti2018,
	title        = {{Generative Adversarial Networks for Unsupervised Monocular Depth Prediction}},
	author       = {Aleotti, Filippo and Tosi, Fabio and Poggi, Matteo and Mattoccia, Stefano},
	year         = 2018,
	month        = sep,
	booktitle    = {Proc. of ECCV - Workshops},
	address      = {Munich, Germany},
	pages        = {1--18},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{Kumar2018a,
	title        = {{Monocular Depth Prediction Using Generative Adversarial Networks}},
	author       = {CS Kumar, Arun and Bhandarkar, Suchendra M. and Prasad, Mukta},
	year         = 2018,
	month        = jun,
	booktitle    = {Proc. of CVPR - Workshops},
	address      = {Salt Lake City, UT, USA},
	pages        = {1--9}
}
@inproceedings{Pilzer2018,
	title        = {{Unsupervised Adversarial Depth Estimation Using Cycled Generative Networks}},
	author       = {Pilzer, Andrea and Xu, Dan and Puscas, Mihai and Ricci, Elisa and Sebe, Nicu},
	year         = 2018,
	month        = sep,
	booktitle    = {Proc. of 3DV},
	address      = {Verona, Italy},
	pages        = {587--595}
}
@inproceedings{Tosi2019,
	title        = {{Learning Monocular Depth Estimation Infusing Traditional Stereo Knowledge}},
	author       = {Tosi, Fabio and Aleotti, Filippo and Poggi, Matteo and Mattoccia, Stefano},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {9799--9809},
	keywords     = {Speech Recognition}
}
@inproceedings{Zhou2019,
	title        = {{Unsupervised High-Resolution Depth Learning From Videos With Dual Networks}},
	author       = {Zhou, Junsheng and Wang, Yuwang and Qin, Kaihuai and Zeng, Wenjun},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {6872--6881},
	keywords     = {Depth Prediction}
}
@inproceedings{Wang2020a,
	title        = {{SDC-Depth: Semantic Divide-and-Conquer Network for Monocular DepthEstimation}},
	author       = {Wang, Lijun and Zhang, Jianming and Wang, Oliver and Lin, Zhe and Lu, Huchuan},
	year         = 2020,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Seattle, WA, USA},
	pages        = {541--550}
}
@inproceedings{Wang2020b,
	title        = {{BiFuse: Monocular 360° Depth Estimation via Bi-Projection Fusion}},
	author       = {Wang, Fu-En and Yeh, Yu-Hsuan and Sun, Min and Chiu, Wei-Chen and Tsai, Yi-Hsuan},
	year         = 2020,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Seattle, WA, USA},
	pages        = {462--471},
	keywords     = {Depth Prediction}
}
@inproceedings{Jin2020,
	title        = {{Geometric Structure Based and Regularized Depth EstimationFrom 360° Indoor Imagery}},
	author       = {Jin, Lei and Xu, Yanyu and Zheng, Jia and Zhang, Junfei and Tang, Rui and Xu, Shugong},
	year         = 2020,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Seattle, WA, USA},
	pages        = {889--898},
	keywords     = {Depth Prediction}
}
@inproceedings{Bozorgtabar2019,
	title        = {{SynDeMo: Synergistic Deep Feature Alignment for Joint Learning of Depth and Ego-Motion}},
	author       = {Bozorgtabar, Behzad and Rad, Mohammad Saeed and Mahapatra, Dwarikanath and Thiran, Jean-Philippe},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {4210--4219},
	keywords     = {Depth Prediction}
}
@inproceedings{Wang2018e,
	title        = {{Learning Depth From Monocular Videos Using Direct Methods}},
	author       = {Wang, Chaoyang and Miguel Buenaposada, Jos\'{e} and Zhu, Rui and Lucey, Simon},
	year         = 2018,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Salt Lake City, UT, USA},
	pages        = {2022--2030},
	keywords     = {Speech Recognition}
}
@inproceedings{Pilzer2019,
	title        = {{Refine and Distill: Exploiting Cycle-Inconsistency and Knowledge Distillation for Unsupervised Monocular Depth Estimation}},
	author       = {Pilzer, Andrea and Lathuiliere, Stephane and Sebe, Nicu and Ricci, Elisa},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {9768--9777},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{yin2018geonet,
	title        = {Geonet: Unsupervised learning of dense depth, optical flow and camera pose},
	author       = {Yin, Zhichao and Shi, Jianping},
	year         = 2018,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {1983--1992}
}
@inproceedings{zou2018df,
	title        = {Df-net: Unsupervised joint learning of depth and flow using cross-task consistency},
	author       = {Zou, Yuliang and Luo, Zelun and Huang, Jia-Bin},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {36--53}
}
@inproceedings{yang2018deep,
	title        = {Deep virtual stereo odometry: Leveraging deep depth prediction for monocular direct sparse odometry},
	author       = {Yang, Nan and Wang, Rui and Stuckler, Jorg and Cremers, Daniel},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {817--833}
}
@inproceedings{klodt2018supervising,
	title        = {Supervising the new with the old: learning SFM from SFM},
	author       = {Klodt, Maria and Vedaldi, Andrea},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {698--713}
}
@article{Khomutenko2016eucm,
	title        = {An Enhanced Unified Camera Model},
	author       = {Bogdan Khomutenko and Gaetan Garcia and Philippe Martinet},
	year         = 2016,
	journal      = {IEEE Robotics and Automation Letters},
	volume       = 1,
	number       = 1,
	pages        = {137--144}
}
@article{herbert1987area,
	title        = {Area projections of fisheye photographic lenses},
	author       = {Herbert, Thomas J},
	year         = 1987,
	journal      = {Agricultural and Forest Meteorology},
	publisher    = {Elsevier},
	volume       = 39,
	number       = {2-3},
	pages        = {215--223}
}
@article{barreto2006unified,
	title        = {Unifying image plane liftings for central catadioptric and dioptric cameras},
	author       = {Barreto, Joao P},
	year         = 2006,
	journal      = {Imaging Beyond the Pinhole Camera},
	publisher    = {Springer},
	pages        = {21–-38}
}
@article{hughes2010fisheye,
	title        = {Accuracy of fish-eye lens models},
	author       = {Ciar\'{a}n Hughes and Patrick Denny and Edward Jones and Martin Glavin},
	year         = 2010,
	journal      = {Applied Optics},
	publisher    = {Optical Society of America},
	volume       = 49,
	number       = 17,
	pages        = {3338--3347}
}
@inproceedings{strand2005fish,
	title        = {Correcting radial distortion by circle fitting},
	author       = {R. Strand and E. Hayman},
	year         = 2005,
	booktitle    = {Proceedings of the 16th British Machine Vision Conference (BMVC)}
}
@inproceedings{cordts2016cityscapes,
	title        = {The cityscapes dataset for semantic urban scene understanding},
	author       = {Cordts, Marius and Omran, Mohamed and Ramos, Sebastian and Rehfeld, Timo and Enzweiler, Markus and Benenson, Rodrigo and Franke, Uwe and Roth, Stefan and Schiele, Bernt},
	year         = 2016,
	booktitle    = {Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages        = {3213--3223}
}
@article{arican2009dense,
	title        = {Dense depth estimation from omnidirectional images},
	author       = {Ar{\i}can, Zafer and Frossard, Pascal},
	year         = 2009
}
@article{zhao2016loss,
	title        = {Loss functions for image restoration with neural networks},
	author       = {Zhao, Hang and Gallo, Orazio and Frosio, Iuri and Kautz, Jan},
	year         = 2016,
	journal      = {IEEE Transactions on Computational Imaging},
	publisher    = {IEEE},
	volume       = 3,
	number       = 1,
	pages        = {47--57}
}
@inproceedings{ronneberger2015u,
	title        = {U-net: Convolutional networks for biomedical image segmentation},
	author       = {Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
	year         = 2015,
	booktitle    = {International Conference on Medical image computing and computer-assisted intervention},
	pages        = {234--241},
	organization = {Springer}
}
@inproceedings{he2016deep,
	title        = {Deep residual learning for image recognition},
	author       = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	year         = 2016,
	booktitle    = {Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages        = {770--778}
}
@inproceedings{zhu2019deformable,
	title        = {Deformable convnets v2: More deformable, better results},
	author       = {Zhu, Xizhou and Hu, Han and Lin, Stephen and Dai, Jifeng},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {9308--9316}
}
@inproceedings{paszke2017automatic,
	title        = {Automatic Differentiation in {PyTorch}},
	author       = {Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
	year         = 2017,
	booktitle    = {NIPS Autodiff Workshop}
}
@article{kingma2014adam,
	title        = {Adam: A method for stochastic optimization},
	author       = {Kingma, Diederik P and Ba, Jimmy},
	year         = 2014,
	journal      = {arXiv preprint arXiv:1412.6980}
}
@inproceedings{ioffe2015batch,
	title        = {Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
	author       = {Ioffe, Sergey and Szegedy, Christian},
	year         = 2015,
	booktitle    = {Proceedings of the 32Nd International Conference on International Conference on Machine Learning - Volume 37},
	location     = {Lille, France},
	publisher    = {JMLR.org},
	series       = {ICML'15},
	pages        = {448--456},
	url          = {http://dl.acm.org/citation.cfm?id=3045118.3045167},
	numpages     = 9,
	acmid        = 3045167
}
@inproceedings{wu2018group,
	title        = {Group normalization},
	author       = {Wu, Yuxin and He, Kaiming},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {3--19}
}
@article{he2018rethinking,
	title        = {Rethinking imagenet pre-training},
	author       = {He, Kaiming and Girshick, Ross and Doll{\'a}r, Piotr},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1811.08883}
}
@article{aitken2017checkerboard,
	title        = {Checkerboard artifact free sub-pixel convolution: A note on sub-pixel convolution, resize convolution and convolution resize},
	author       = {Aitken, Andrew and Ledig, Christian and Theis, Lucas and Caballero, Jose and Wang, Zehan and Shi, Wenzhe},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1707.02937}
}
@inproceedings{eigen2015predicting,
	title        = {{Predicting Depth, Surface Normals and Semantic Labels With a Common Multi-Scale Convolutional Architecture}},
	author       = {Eigen, David and Fergus, Rob},
	year         = 2015,
	month        = dec,
	booktitle    = {Proc. of ICCV},
	address      = {Santiago, Chile},
	pages        = {2650--2658},
	keywords     = {Depth Prediction; Semantic Segmentation; Optical Flow, Speech Recognition}
}
@article{liu2015learning,
	title        = {Learning depth from single monocular images using deep convolutional neural fields},
	author       = {Liu, Fayao and Shen, Chunhua and Lin, Guosheng and Reid, Ian},
	year         = 2015,
	journal      = {IEEE transactions on pattern analysis and machine intelligence},
	publisher    = {IEEE},
	volume       = 38,
	number       = 10,
	pages        = {2024--2039}
}
@inproceedings{nath2018adadepth,
	title        = {Adadepth: Unsupervised content congruent adaptation for depth estimation},
	author       = {Nath Kundu, Jogendra and Krishna Uppala, Phani and Pahuja, Anuj and Venkatesh Babu, R},
	year         = 2018,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {2656--2665}
}
@inproceedings{yang2018unsupervised,
	title        = {Unsupervised learning of geometry from videos with edge-aware depth-normal consistency},
	author       = {Yang, Zhenheng and Wang, Peng and Xu, Wei and Zhao, Liang and Nevatia, Ramakant},
	year         = 2018,
	booktitle    = {Thirty-Second AAAI Conference on Artificial Intelligence}
}
@inproceedings{yang2018lego,
	title        = {Lego: Learning edge with geometry all at once by watching videos},
	author       = {Yang, Zhenheng and Wang, Peng and Wang, Yang and Xu, Wei and Nevatia, Ram},
	year         = 2018,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {225--234}
}
@inproceedings{ranjan2019competitive,
	title        = {Competitive Collaboration: Joint Unsupervised Learning of Depth, Camera Motion, Optical Flow and Motion Segmentation},
	author       = {Ranjan, Anurag and Jampani, Varun and Balles, Lukas and Kim, Kihwan and Sun, Deqing and Wulff, Jonas and Black, Michael J},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {12240--12249}
}
@inproceedings{KITTIDepth,
	title        = {Are We Ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
	author       = {Geiger, Andreas},
	year         = 2012,
	booktitle    = {Proceedings of the 2012 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	publisher    = {IEEE Computer Society},
	address      = {Washington, DC, USA},
	series       = {CVPR '12},
	pages        = {3354--3361},
	isbn         = {978-1-4673-1226-4},
	url          = {http://dl.acm.org/citation.cfm?id=2354409.2354978},
	numpages     = 8,
	acmid        = 2354978,
	keywords     = {Benchmark testing,Cameras,Optical imaging,Visualization,Optical sensors,Measurement}
}
@article{li2017dense,
	title        = {Dense transformer networks},
	author       = {Li, Jun and Chen, Yongjun and Cai, Lei and Davidson, Ian and Ji, Shuiwang},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1705.08881}
}
@inproceedings{pillai2019superdepth,
	title        = {Superdepth: Self-supervised, super-resolved monocular depth estimation},
	author       = {Pillai, Sudeep and Ambru{\c{s}}, Rare{\c{s}} and Gaidon, Adrien},
	year         = 2019,
	booktitle    = {2019 International Conference on Robotics and Automation (ICRA)},
	pages        = {9250--9256},
	organization = {IEEE}
}
@inproceedings{zhan2018unsupervised,
	title        = {Unsupervised learning of monocular depth estimation and visual odometry with deep feature reconstruction},
	author       = {Zhan, Huangying and Garg, Ravi and Saroj Weerasekera, Chamara and Li, Kejie and Agarwal, Harsh and Reid, Ian},
	year         = 2018,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {340--349}
}
@inproceedings{su2018kernel,
	title        = {Kernel transformer networks for compact spherical convolution},
	author       = {Su, Yu-Chuan and Grauman, Kristen},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages        = {9442--9451}
}
@inproceedings{kukelova2015radial,
	title        = {Radial distortion homography},
	author       = {Kukelova, Zuzana and Heller, Jan and Bujnak, Martin and Pajdla, Tomas},
	year         = 2015,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	pages        = {639--647}
}
@inproceedings{coors2018spherenet,
	title        = {{SphereNet}: {L}earning spherical representations for detection and classification in omnidirectional images},
	author       = {Coors, Benjamin and Paul Condurache, Alexandru and Geiger, Andreas},
	year         = 2018,
	booktitle    = {Proceedings of the European Conference on Computer Vision (ECCV)},
	pages        = {518--533}
}
@inproceedings{uhrig2017sparsity,
	title        = {{Sparsity Invariant CNNs}},
	author       = {Uhrig, Jonas and Schneider, Nick and Schneider, Lukas and Franke, Uwe and Brox, Thomas and Geiger, Andreas},
	year         = 2017,
	month        = oct,
	booktitle    = {Proc. of 3DV},
	address      = {Verona, Italy},
	pages        = {11--20},
	keywords     = {Speech Recognition}
}
@inproceedings{deng2009imagenet,
	title        = {Imagenet: A large-scale hierarchical image database},
	author       = {Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
	year         = 2009,
	booktitle    = {2009 IEEE conference on computer vision and pattern recognition},
	pages        = {248--255},
	organization = {Ieee}
}
@inproceedings{Zhang2019a,
	title        = {{Pattern-Affinitive Propagation Across Depth, Surface Normal and Semantic Segmentation}},
	author       = {Zhang, Zhenyu and Cui, Zhen and Xu, Chunyan and Yan, Yan and Sebe, Nicu and Yang, Jian},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {4106--4115}
}
@inproceedings{Ochs2019,
	title        = {{SDNet: Semantically Guided Depth Estimation Network}},
	author       = {Ochs, Matthias and Kretz, Adrian and Mester, Rudolf},
	year         = 2019,
	month        = sep,
	booktitle    = {Proc. of GCPR},
	address      = {Dortmund, Germany},
	pages        = {288--302},
	keywords     = {Depth Prediction; Domain Adaptation}
}
@inproceedings{Zhao2019,
	title        = {{Geometry-Aware Symmetric Domain Adaptation for Monocular Depth Estimation}},
	author       = {Zhao, Shanshan and Fu, Huan and Gong, Mingming and Tao, Dacheng},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	keywords     = {Domain Adaptation}
}
@inproceedings{Kirillov2019,
	title        = {{Panoptic Feature Pyramid Networks}},
	author       = {Alexander Kirillov and Ross Girshick and Kaiming He and Piotr Doll{\'{a}}r},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {6399--6408},
	keywords     = {Semantic Segmentation; Instance Segmentation, Speech Recognition}
}
@inproceedings{Liu2019,
	title        = {{SelFlow: Self-Supervised Learning of Optical Flow}},
	author       = {Liu, Pengpeng and Lyu, Michael and King, Irwin and Xu, Jia},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {4571--4580},
	keywords     = {Optical Flow}
}
@inproceedings{Rhe2017,
	title        = {{Unsupervised Deep Learning for Optical Flow Estimation}},
	author       = {Ren, Zhe and Yan, Junchi and Ni, Bingbing and Liu, Bin and Yang, Xiaokang and Zha, Hongyuan},
	year         = 2017,
	month        = feb,
	booktitle    = {Proc. of AAAI},
	address      = {San Francisco, CA, USA},
	pages        = {1495--1501},
	keywords     = {Optical Flow}
}
@inproceedings{Wang2019c,
	title        = {{UnOS: Unified Unsupervised Optical-Flow and Stereo-Depth Estimation by Watching Videos}},
	author       = {Wang, Yang and Wang, Peng and Yang, Zhenheng and Luo, Chenxu and Yang, Yi and Xu, Wei},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {8071--8081},
	keywords     = {Depth Estimation, Optical Flow}
}
@inproceedings{Yang2018c,
	title        = {{Every Pixel Counts: Unsupervised Geometry Learning With Holistic 3D Motion Understanding}},
	author       = {Yang, Zhenheng and Wang, Peng and Wang, Yang and Xu, Wei and Nevatia, Ram},
	year         = 2018,
	month        = sep,
	booktitle    = {Proc. of ECCV - Workshops},
	address      = {Munich, Germany},
	pages        = {1--17},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{Liu2019a,
	title        = {{Unsupervised Learning of Scene Flow Estimation Fusing With Local Rigidity}},
	author       = {Liu, Liang and Zhai, Guangyao and Ye, Wenlong and Liu, Yong},
	year         = 2019,
	month        = aug,
	booktitle    = {Proc. of IJCAI},
	address      = {Macao, China},
	pages        = {876--882},
	keywords     = {Depth Prediction; Optical Flow}
}
@inproceedings{Chen2019b,
	title        = {{Self-Supervised Learning With Geometric Constraints in Monocular Video Connecting Flow, Depth, and Camera}},
	author       = {Chen, Yuhua and Schmid, Cordelia and Sminchisescu, Cristian},
	year         = 2019,
	month        = oct,
	booktitle    = {Proc. of ICCV},
	address      = {Seoul, Korea},
	pages        = {7063--7072},
	keywords     = {Depth Prediction}
}
@article{Luo2019a,
	title        = {Every Pixel Counts ++: Joint Learning of Geometry and Motion with 3D Holistic Understanding},
	author       = {C. {Luo} and Z. {Yang} and P. {Wang} and Y. {Wang} and W. {Xu} and R. {Nevatia} and A. {Yuille}},
	year         = 2020,
	journal      = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	volume       = 42,
	number       = 10,
	pages        = {2624--2641}
}
@inproceedings{Li2019,
	title        = {{Learning the Depths of Moving People by Watching Frozen People}},
	author       = {Li, Zhengqi and Dekel, Tali and Cole, Forrester and Tucker, Richard and Snavely, Noah and Liu, Ce and Freeman, William T.},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {4521--4530},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{Yin2018,
	title        = {{GeoNet: Unsupervised Learning of Dense Depth, Optical Flow and Camera Pose}},
	author       = {Yin, Zhichao and Shi, Jianping},
	year         = 2018,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Salt Lake City, UT, USA},
	pages        = {1983--1992},
	keywords     = {Depth Prediction}
}
@inproceedings{Chen2019a,
	title        = {{Towards Scene Understanding: Unsupervised Monocular Depth Estimation With Semantic-Aware Representation}},
	author       = {Chen, Po-Yi and Liu, Alexander H. and Liu, Yen-Cheng and Wang, Yu-Chiang F.},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {2624--2632},
	keywords     = {Depth Prediction; Semantic Segmentation, Speech Recognition}
}
@inproceedings{Novosel2019,
	title        = {{Boosting Semantic Segmentation With Multi-Task Self-Supervised Learning for Autonomous Driving Applications}},
	author       = {Novosel, Jelena and Viswanath, Prashanth and Arsenali, Bruno},
	year         = 2019,
	month        = dec,
	booktitle    = {Proc. of NeurIPS - Workshops},
	address      = {Vancouver, BC, Canada},
	pages        = {1--11},
	keywords     = {Semantic Segmentation, Depth Prediction}
}
@inproceedings{Yang2018b,
	title        = {{SegStereo: Exploiting Semantic Information for Disparity Estimation}},
	author       = {Yang, Guorun and Zhao, Hengshuang and Shi, Jianping and Deng, Zhidong and Jia, Jiaya},
	year         = 2018,
	month        = sep,
	booktitle    = {Proc. of ECCV},
	address      = {Munich, Germany},
	pages        = {636--651},
	keywords     = {Depth Prediction; Semantic Segmentation, Speech Recognition}
}
@inproceedings{Casser2019,
	title        = {{Depth Prediction Without the Sensors: Leveraging Structure for Unsupervised Learning from Monocular Videos}},
	author       = {Casser, Vincent and Pirk, Soeren and Mahjourian, Reza and Angelova, Anelia},
	year         = 2019,
	month        = jan,
	booktitle    = {Proc. of AAAI},
	address      = {Honolulu, HI, USA},
	pages        = {8001--8008},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{Zhu2020,
	title        = {{The Edge of Depth: Explicit Constraints between Segmentation and Depth}},
	author       = {Zhu, Shengjie and Brazil, Garrick and Liu, Xiaoming},
	year         = 2020,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Seattle, WA, USA},
	pages        = {13116--13125},
	keywords     = {Depth Prediction}
}
@inproceedings{Casser2019a,
	title        = {{Unsupervised Monocular Depth and Ego-Motion Learning With Structure and Semantics}},
	author       = {Casser, Vincent and Pirk, Soeren and Mahjourian, Reza and Angelova, Anelia},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR - Workshops},
	address      = {Long Beach, CA, USA},
	pages        = {1--8}
}
@inproceedings{Godard2017,
	title        = {{Unsupervised Monocular Depth Estimation With Left-Right Consistency}},
	author       = {Godard, Cl{\'e}ment and Mac Aodha, Oisin and Brostow, Gabriel J.},
	year         = 2017,
	month        = jul,
	booktitle    = {Proc. of CVPR},
	address      = {Honolulu, HI, USA},
	pages        = {270--279},
	keywords     = {Depth Prediction}
}
@inproceedings{Fu2018,
	title        = {{Deep Ordinal Regression Network for Monocular Depth Estimation}},
	author       = {Fu, Huan and Gong, Mingming and Wang, Chaohui and Batmanghelich, Kayhan and Tao, Dacheng},
	year         = 2018,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Salt Lake City, UT, USA},
	pages        = {2002--2011},
	keywords     = {Depth Prediction, Speech Recognition}
}
@inproceedings{Zhang2019b,
	title        = {{GA-Net: Guided Aggregation Net for End-to-End Stereo Matching}},
	author       = {Zhang, Feihu and Prisacariu, Victor and Yang, Ruigang and Torr, Philip H. S.},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {185--194},
	keywords     = {Depth Prediction}
}
@article{Vijayanarasimhan2017,
	title        = {SfM-Net: Learning of Structure and Motion from Video},
	author       = {Sudheendra Vijayanarasimhan and S. Ricco and C. Schmid and R. Sukthankar and K. Fragkiadaki},
	year         = 2017,
	journal      = {ArXiv},
	volume       = {abs/1704.07804}
}
@inproceedings{Meng2019a,
	title        = {{SIGNet: Semantic Instance Aided Unsupervised 3D Geometry Perception}},
	author       = {Meng, Yue and Lu, Yongxi and Raj, Aman and Sunarjo, Samuel and Guo, Rui and Javidi, Tara and Bansal, Gaurav and Bharadia, Dinesh},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {9810--9820},
	keywords     = {Depth Prediction, Semantic Segmentation}
}
@inproceedings{Ranjan2019,
	title        = {{Competitive Collaboration: Joint Unsupervised Learning of Depth, Camera Motion, Optical Flow and Motion Segmentation}},
	author       = {Ranjan, Anurag and Jampani, Varun and Balles, Lukas and Kim, Kihwan and Sun, Deqing and Wulff, Jonas and Black, Michael J.},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {12240--12249},
	keywords     = {Depth Prediction, Semantic Segmentation}
}
@inproceedings{chennupati2019multinet++,
	title        = {Multinet++: Multi-stream feature aggregation and geometric loss strategy for multi-task learning},
	author       = {Chennupati, Sumanth and Sistu, Ganesh and Yogamani, Senthil and A Rawashdeh, Samir},
	year         = 2019,
	booktitle    = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
	pages        = {0--0}
}
@inproceedings{sistu2019neurall,
	title        = {NeurAll: Towards a Unified Visual Perception Model for Automated Driving},
	author       = {Sistu, Ganesh and Leang, Isabelle and Chennupati, Sumanth and Yogamani, Senthil and Hughes, Ciar{\'a}n and Milz, Stefan and Rawashdeh, Samir},
	year         = 2019,
	booktitle    = {2019 IEEE Intelligent Transportation Systems Conference (ITSC)},
	pages        = {796--803},
	organization = {IEEE}
}
@conference{chennupati2019auxnet,
	title        = {AuxNet: Auxiliary Tasks Enhanced Semantic Segmentation for Automated Driving},
	author       = {Sumanth Chennupati and Ganesh Sistu and Senthil Yogamani and Samir Rawashdeh},
	year         = 2019,
	booktitle    = {Proceedings of the 14th International Joint Conference on Computer Vision, Imaging and Computer Graphics Theory and Applications (VISAPP)},
	pages        = {645--652}
}
@inproceedings{kumar2018monocular,
	title        = {Monocular fisheye camera depth estimation using sparse lidar supervision},
	author       = {Kumar, Varun Ravi and Milz, Stefan and Witt, Christian and Simon, Martin and Amende, Karl and Petzold, Johannes and Yogamani, Senthil and Pech, Timo},
	year         = 2018,
	booktitle    = {2018 21st International Conference on Intelligent Transportation Systems (ITSC)},
	pages        = {2853--2858},
	organization = {IEEE}
}
@inproceedings{Guizilini2020,
	title        = {{Semantically-Guided Representation Learning for Self-Supervised Monocular Depth}},
	author       = {Guizilini, Vitor and Hou, Rui and Li, Jie and Ambrus, Rares and Gaidon, Adrien},
	year         = 2020,
	month        = apr,
	booktitle    = {Proc. of ICLR},
	address      = {Addis Ababa, Ethiopia},
	pages        = {1--14}
}
@inproceedings{Kendall2018,
	title        = {{Multi-Task Learning Using Uncertainty to Weigh Losses for Scene Geometry and Semantics}},
	author       = {Kendall, Alex and Gal, Yarin and Cipolla, Roberto},
	year         = 2018,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Salt Lake City, UT, USA},
	pages        = {7482--7491},
	keywords     = {Depth Prediction Semantic Segmentation}
}
@inproceedings{Chen2018d,
	title        = {{GradNorm: Gradient Normalization for Adaptive Loss Balancing in Deep Multitask Networks}},
	author       = {Chen, Zhao and Badrinarayanan, Vijay and Lee, Chen-Yu and Rabinovich, Andrew},
	year         = 2018,
	month        = jul,
	booktitle    = {Proc. of ICML},
	address      = {Stockholm, Sweden},
	pages        = {794--803}
}
@inproceedings{Ganin2015,
	title        = {{Unsupervised Domain Adaptation by Backpropagation}},
	author       = {Ganin, Yaroslav and Lempitsky, Victor},
	year         = 2015,
	month        = jul,
	booktitle    = {Proc. of ICML},
	address      = {Lille, France},
	pages        = {1180--1189},
	keywords     = {Computer Vision; Domain Adaptation}
}
@inproceedings{Bolte2019a,
	title        = {{Unsupervised Domain Adaptation to Improve Image Segmentation Quality Both in the Source and Target Domain}},
	author       = {Bolte, Jan-Aike and Kamp, Markus and Breuer, Antonia and Homoceanu, Silviu and Schlicht, Peter and Huger, Fabian and Lipinski, Daniel and Fing\-scheidt, Tim},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR - Workshops},
	address      = {Long Beach, CA, USA},
	pages        = {1--10},
	keywords     = {Domain Adaptation}
}
@inproceedings{Klingner2020,
	title        = {{Improved Noise and Attack Robustness for Semantic Segmentation by Using Multi-Task Training with Self-Supervised Depth Estimation}},
	author       = {Klingner, Marvin and B\"{a}r, Andreas and Fing\-scheidt, Tim},
	year         = 2020,
	month        = jun,
	booktitle    = {Proc. of CVPR - Workshops},
	address      = {Seattle, WA, USA},
	pages        = {1--11},
	keywords     = {Depth Estimation, Semantic Segmentation}
}
@inproceedings{zhang2019lookahead,
	title        = {Lookahead Optimizer: k steps forward, 1 step back},
	author       = {Zhang, Michael and Lucas, James and Ba, Jimmy and Hinton, Geoffrey E},
	year         = 2019,
	booktitle    = {Advances in Neural Information Processing Systems},
	pages        = {9593--9604}
}
@article{liu2019variance,
	title        = {On the variance of the adaptive learning rate and beyond},
	author       = {Liu, Liyuan and Jiang, Haoming and He, Pengcheng and Chen, Weizhu and Liu, Xiaodong and Gao, Jianfeng and Han, Jiawei},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1908.03265}
}
@inproceedings{smith2019super,
	title        = {Super-convergence: Very fast training of neural networks using large learning rates},
	author       = {Smith, Leslie N and Topin, Nicholay},
	year         = 2019,
	booktitle    = {Artificial Intelligence and Machine Learning for Multi-Domain Operations Applications},
	volume       = 11006,
	pages        = 1100612,
	organization = {International Society for Optics and Photonics}
}
@inproceedings{kumar2020fisheyedistancenet,
  title        = {Fisheyedistancenet: Self-supervised scale-aware distance estimation using monocular fisheye camera for autonomous driving},
  author       = {Kumar, Varun Ravi and Hiremath, Sandesh Athni and Bach, Markus and Milz, Stefan and Witt, Christian and Pinard, Cl{\'e}ment and Yogamani, Senthil and M{\"a}der, Patrick},
  year         = 2020,
  booktitle    = {2020 IEEE International Conference on Robotics and Automation (ICRA)},
  pages        = {574--581},
  organization = {IEEE}
}
@article{russakovsky2015imagenet,
	title        = {Imagenet large scale visual recognition challenge},
	author       = {Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
	year         = 2015,
	journal      = {International journal of computer vision},
	publisher    = {Springer},
	volume       = 115,
	number       = 3,
	pages        = {211--252}
}
@inproceedings{barron2019general,
	title        = {{A General and Adaptive Robust Loss Function}},
	author       = {Barron, Jonathan T.},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {4331--4339}
}
@inproceedings{su2019pixel,
	title        = {{Pixel-Adaptive Convolutional Neural Networks}},
	author       = {Su, Hang and Jampani, Varun and Sun, Deqing and Gallo, Orazio and Learned-Miller, Erik and Kautz, Jan},
	year         = 2019,
	month        = jun,
	booktitle    = {Proc. of CVPR},
	address      = {Long Beach, CA, USA},
	pages        = {11166--11175}
}
@article{ramachandran2019stand,
	title        = {Stand-alone self-attention in vision models},
	author       = {Ramachandran, Prajit and Parmar, Niki and Vaswani, Ashish and Bello, Irwan and Levskaya, Anselm and Shlens, Jonathon},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1906.05909}
}
@inproceedings{klingner2020selfsupervised,
	title        = {{Self-Supervised Monocular Depth Estimation: Solving the Dynamic Object Problem by Semantic Guidance}},
	author       = {Klingner, Marvin and Termöhlen, Jan-Aike and Mikolajczyk, Jonas and Fingscheidt, Tim},
	year         = 2020,
	month        = aug,
	booktitle    = {Proc. of ECCV},
	address      = {Glasgow, UK}
}
@inproceedings{vaswani2017attention,
	title        = {Attention is all you need},
	author       = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
	year         = 2017,
	month        = dec,
	booktitle    = {Proc. of NIPS},
	address      = {Long Beach, CA, USA},
	pages        = {5998--6008}
}
@inproceedings{kumar2020unrectdepthnet,
	title        = {UnRectDepthNet: Self-Supervised Monocular Depth Estimation using a Generic Framework for Handling Common Camera Distortion Models},
	author       = {Ravi Kumar, Varun and Yogamani, Senthil and Bach, Markus and Witt, Christian and Milz, Stefan and Mader, Patrick},
	year         = 2020,
	booktitle    = {International Conference on Intelligent Robots and Systems (IROS)}
}
